Deep Incremental Learning of Imbalanced Data for Just-In-Time Software Defect Prediction

This work stems from three observations on prior Just-In-Time Software Defect Prediction (JIT-SDP) models. First, prior studies treat the JIT-SDP problem solely as a classification problem. Second, prior JIT-SDP studies do not consider that class balancing processing may change the underlying characteristics of software changeset data. Third, only a single source of concept drift, the class imbalance evolution is addressed in prior JIT-SDP incremental learning models. We propose an incremental learning framework called CPI-JIT for JIT-SDP. First, in addition to a classification modeling component, the framework includes a time-series forecast modeling component in order to learn temporal interdependent relationship in the changesets. Second, the framework features a purposefully designed over-sampling balancing technique based on SMOTE and Principal Curves called SMOTE-PC. SMOTE-PC preserves the underlying distribution of software changeset data. In this framework, we propose an incremental deep neural network model called DeepICP. Via an evaluation using \numprojs software projects, we show that: 1) SMOTE-PC improves the model's predictive performance; 2) to some software projects it can be beneficial for defect prediction to harness temporal interdependent relationship of software changesets; and 3) principal curves summarize the underlying distribution of changeset data and reveals a new source of concept drift that the DeepICP model is proposed to adapt to.

==> baseline.tex <==
\subsection{Research Baseline}
The performance of Kamei et al.'s defect proness logistic regression (DPLR)
prediction model is in Table~\ref{tab:baseline:kamei2012:dp}

\begin{table*}
	\caption{Comparison of the predictive performance of the replicated defect
	proneness prediction model and the original results in Kamei et
	al.~\cite{kamei2012large}}
	\label{tab:baseline:kamei2012:dp}
	\begin{tabular}{l l l l l l l l l l l}
		\multirow{2}{*}{Project} 
			& \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{Precision} & \multicolumn{2}{c}{Recall} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{AUC-ROC} \\
			& Original & Baseline   & Original & Baseline  & Original & Baseline & Original & Baseline & Original & Baseline \\
	Bugzilla & 0.67 & $0.669 \pm 0.025$ & 0.54 &$0.539 \pm 0.045$ &0.69 &$0.681 \pm 0.053$ &0.60 &$0.601 \pm 0.040$ &0.74 &$0.740 \pm 0.031$ \\
	Columba  & 0.70 & $0.708 \pm 0.222$ & 0.51 &$0.516 \pm 0.045$ &0.67 &$0.656 \pm 0.048$ &0.58 &$0.577 \pm 0.045$ &0.75 &$0.758 \pm 0.028$ \\
	JDT      & 0.69 & $0.691 \pm 0.008$ & 0.26 &$0.266 \pm 0.011$ &0.65 &$0.651 \pm 0.013$ &0.37 &$0.378 \pm 0.011$ &0.74 &$0.736 \pm 0.008$ \\
	Mozilla  & 0.77 & $0.767 \pm 0.007$ & 0.13 &$0.135 \pm 0.008$ &0.63 &$0.641 \pm 0.020$ &0.22 &$0.224 \pm 0.012$ &0.77 &$0.775 \pm 0.009$ \\
	Platform & 0.67 & $0.672 \pm 0.005$ & 0.27 &$0.267 \pm 0.007$ &0.70 &$0.701 \pm 0.021$ &0.38 &$0.386 \pm 0.012$ &0.75 &$0.751 \pm 0.001$ \\
	Postgres & 0.74 & $0.749 \pm 0.008$ & 0.49 &$0.500 \pm 0.002$ &0.65 &$0.650 \pm 0.021$ &0.56 &$0.565 \pm 0.018$ &0.79 &$0.790 \pm 0.013$ \\
	\end{tabular}
\end{table*}


The performance of Kamei et al.'s effort-aware linear regression (EALR)
prediction is in Table~\ref{tab:baseline:kamei2012:ea}

\begin{table}
	\caption{Comparison of the predictive performance of the replicated
	effort-aware prediction model and the original results in Kamei et
	al.~\cite{kamei2012large}}
	\label{tab:baseline:kamei2012:dp}
	\begin{tabular}{l l l l l}
		\multirow{2}{*}{Project} 
			& \multicolumn{2}{c}{Recall@20\%} & \multicolumn{2}{c}{$P_{opt}$} \\
			& Original & Baseline   & Original & Baseline  \\
		Bugzilla & 0.38 & $0.43 \pm 0.11$ & 0.72 & $0.72 \pm 0.07$ \\
		Columba & 0.39 & $0.39 \pm 0.10$ & 0.57 & $0.60 \pm 0.07$ \\
		JDT & 0.20 & $0.19 \pm 0.09$ & 0.48 & $0.46 \pm 0.09$ \\
		Mozilla & 0.15 & $0.15 \pm 0.02$ & 0.45 & $0.45 \pm 0.02$ \\
		Platform & 0.30 & $0.30 \pm 0.09$ & 0.55 & $0.54 \pm 0.03$ \\
		Postgres & 0.26 & $0.28 \pm 0.05$ & 0.51 & $0.51 \pm 0.07$ \\
		Average & 0.28 & $0.29 \pm 0.13$ & 0.55 &  $0.55 \pm 0.11$\\
	\end{tabular}
\end{table}

